Object-Centric Dexterous Manipulation from Human Motion Data

Manipulating objects to achieve desired goal states is a basic but important skill for dexterous manipulation. Human hand motions demonstrate proficient manipulation capability, providing valuable data for training robots with multi-finger hands. Despite this potential, substantial challenges arise due to the embodiment gap between human and robot hands. In this work, we introduce a hierarchical policy learning framework that uses human hand motion data for training object-centric dexterous robot manipulation. At the core of our method is a high-level trajectory generative model, learned with a large-scale human hand motion capture dataset, to synthesize human-like wrist motions conditioned on the desired object goal states. Guided by the generated wrist motions, deep reinforcement learning is further used to train a low-level finger controller that is grounded in the robot's embodiment to physically interact with the object to achieve the goal. Through extensive evaluation across 10 household objects, our approach not only demonstrates superior performance but also showcases generalization capability to novel object geometries and goal states. Furthermore, we transfer the learned policies from simulation to a real-world bimanual dexterous robot system, further demonstrating its applicability in real-world scenarios. Project website: https://cypypccpy.github.io/obj-dex.github.io/.

==> previous_exp/5_experiment_setups.tex <==
\section{Experiment Setups}

\textbf{Tasks.} To validate the performance and generalization capability of the learned policy, we introduce four types of experiment tasks: (1). \textit{Trained}: Both the objects and the desired object goal trajectories are included in the training data. (2). \textit{Unseen Traj}: The objects are from the training set while the goal trajectories are not covered by the training set. (3). \textit{Unseen Obj}: The objects are not included in the training set while the goal trajectories are within the training set. (4). \textit{}

In our experiments, we have three types of the experiment. The first type is ``individual object'', where we select one trajectory for each object in the ARCTIC dataset and train the model for each trajectory. The second type is ``Multi Traj'', involving training a single model on the training set and testing it on the unseen trajectories set. The third type is ``Multi Obj'', involving training a single model on the training set and testing it on the unseen object set. To validate the performance of the high-level planner separately, we train a high-level planner on the training set and test it on the unseen trajectories set and unseen object set.


% Our task is defined as manipulating the object following a sequence of object pose using bimanual dexterous hands. We use the objects' trajectories in the ARCTIC dataset as the desired object trajectories in our experiments. ARCTIC dataset has ten objects, each with approximately 20 trajectories. We select the laptop in the ARCTIC dataset as the unseen object set and take four trajectories randomly for each of the remaining objects as the unseen trajectories set. All the remaining objects' trajectories constitute our training set. In our experiments, we have three types of tasks. The first type is ``individual object'', where we select one trajectory for each object in the ARCTIC dataset and train the model for each trajectory. The second type is ``Multi Traj'', involving training a single model on the training set and testing it on the unseen trajectories set. The third type is ``Multi Obj'', involving training a single model on the training set and testing it on the unseen object set. To validate the performance of the high-level planner separately, we train a high-level planner on the training set and test it on the unseen trajectories set and unseen object set.



% Our experiments aim to achieve the bimanual manipulation tasks demonstrated in the ARCTIC~\cite{fan2023arctic} dataset. Moreover, it should be noted that our method can be applied not only ARCTIC but also other motion capture datasets. In simulations, we utilize two UR10e robotic arms equipped with two dexterous hands in an abreast configuration. Our framework support four different dexterous multi-finger hands: Shadow Hand, Allegro Hand, Schunk Hand, and Ability Hand. Unless otherwise stated, we employed the Shadow Hand in our simulation experiments. Detailed information about the other datasets and other hands are available in the Appendix~\ref{app:other_hands}. In the real world, we use two UR10e robotic arms paired with two Shadow Hands to validate our sim-to-real transfer capability. The experimental setups are depicted in Figure.\ref{fig:workspace}. trained data, unseen data, traj, geo. aim. three type of task. trained, unseen traj not obser, unseen obj. geo

\textbf{Metrics:} 
% For high-level planner, our success metric is the root \textbf{Translation Error (TE)} computed using Euclidean distance in centimeters and \textbf{Orientation Error (OE)} defined by the Frobenius norm of the difference between the rotation matrix. For low-level controller, our success metric is the \textbf{Completion Rate}, which is the percentage of the object trajectory that keeping within the tolerate. The tolerate of the position error is $5cm$ and the tolerate of the rotation error is $0.5rad$. Each motion capture trajectory have a total of 500 steps. Each motion capture trajectory have a total of 500 steps. compare to the ARCTIC, only if, always smaller than. Multi Traj. Multi Obj
For the high-level planner, our metric is the distance between the current pose of the object and the target pose. For position, we use \textbf{Translation Error (TE)}, computed using Euclidean distance in centimeters. For rotation, we use \textbf{Orientation Error (OE)}, defined by the Frobenius norm of the difference between the rotation matrices.
For the low-level controller, our metric is the \textbf{Completion Rate}, which is the percentage of the object trajectory completed only if the object's pose error is smaller than a threshold. The threshold for position is $5$ centimeters and the threshold for rotation is $0.5$ radian. Each motion capture trajectory has a total of 500 steps.


\textbf{Baselines:} We adopted several approaches in our tasks as the baselines. \textbf{Joint-Space Retargeting:} We adopt the joint-space retargeting methods from DexMV~\cite{qin2022dexmv} to transfer the hand motion from ARCTIC to robot hands. \textbf{Fingertip-Space Retargeting:} We directly match the fingertips position of the robot hands to the fingertips position of the human hands in ARCTIC using Inverse Kinematics (IK). \textbf{Ours with Fingertip Reward (Ours w. FR):} Add an additional reward in our framework that makes the positions of the robot's fingertips closer to the human's fingertips. \textbf{Vanilla RL:} Train the RL to learn the motions of the arm and hand together without the hierarchy structure. \textbf{Ours without DAL (Ours w.o. DAL):} Our framework does not involve Data Augmentation Loop. All the reinforcement learning training uses the PPO algorithm in IsaacGym~\cite{} with a NVIDIA RTX3090 GPU.

% \textbf{Questions:} Our experiment primarily seeks to address the following questions: \textbf{Q1:} How effectively can we transfer human motion capture data to dexterous robotic hands? \textbf{Q2:} Can we use a single policy to retarget multiple trajectories and generalize to unseen trajectories? \textbf{Q3:} Can we use a single policy to retarget trajectories involving multiple objects and generalize to unseen objects? \textbf{Q4:} Does utilizing fingertip information help in task-level retargeting? \textbf{Q5:} What effect does Planner-Controller Improvement Loop in DexMimic? \textbf{Q6:} How well does our method perform on dexterous robotic hands other than the Shadow Hand? \textbf{Q7:} Can our policy be transferred from simulation to real-world robots?





==> previous_exp/6_results.tex <==
\section{Results}

\input{table_1}
\input{table_3}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/qual_result_v2.pdf}
    \caption{Qualitative and quantitative analysis. \textbf{(a)} Visualization of the human data, baselines, and our framework. The object that can continue to follow the target is framed in green, and the failure is framed in red. \textbf{(b)} Ablation study of the Data Augmentation Loop. The x-axis is the randomization type of the task, and the y-axis is the completion rate of the task. \textbf{(c)} Ablation study of the type of hands. The x-axis is the type of the hand in the task, and the y-axis is the degree of completion of the task.}
    \label{fig:pull}
    % \vspace{-15pt}
\end{figure*}

\textbf{Q1: How effectively can we transfer human motion capture data to dexterous robotic hands?}
In Table 1, our method consistently outperforms the baseline algorithms with more than 40\%. Additionally, our completion rates exceed 80\%, indicating our proficiency in challenging manipulation tasks. Notably, we observed that manipulations involving larger objects (e.g. box, laptop) typically have higher completion rates, whereas smaller objects (e.g. scissors, phone) have lower success rates. This highlights the ongoing challenge of precisely manipulating small-size objects. Furthermore, the low completion rates for Fingertip IK and Joint Space IK indicate that our tasks are highly dynamic. This is because the more dynamic and contact-intensive the tasks are, the more pronounced the embodiment gap becomes. This would make traditional IK methods largely ineffective.

\textbf{Q2: Can we use a single policy to retarget multiple trajectories/objects and generalize to unseen trajectories/objects?}
In Table 4 Multi Traj row, we explored training a single policy for task-level retargeting across multiple trajectories using the Box object. The policy is trained on 12 different trajectories and testing to 4 unseen trajectories. Our algorithm successfully retarget multiple trajectories, achieving 70\% completion rates and demonstrated good generalization on unseen trajectories with 50\% completion rates. In Table 4 Multi Obj row, we investigated training a single policy to simultaneously complete multiple trajectories for multiple objects in task-level retargeting. This proved to be a challenging task, achieving only an average completion rate of 45\% in trained objects and 22\% in unseen objects. Thus, we find that generalizing across the object geometry in task-level retargeting is difficult.

\textbf{Q3: How does the error of the wrist trajectory generated by high-level planner compare to the ARCTIC dataset?}
In Table 2, we tested three different network architectures—MLP, RNN, and Transformer—in the ARCTIC dataset. The results show that the BC-Trans performed the best, with a low level of the cumulative Transition Error and Orientation Error. This demonstrates that our high-level planner can accurately generate reference wrist trajectories and generalize to unseen trajectories and category-level unseen objects. Visualizations of the high-level planner can be found in the Appendix.

\textbf{Q4: Does utilizing fingertip information help in task-level retargeting?}
In Table 1 and Table 4, the addition of fingertip rewards resulted in a decrease in performance compared to our method, with respective decreases of 40\% and 30\%. We attribute this phenomenon to inaccuracies in fingertip information when there is a embodiedment gap. As mentioned in \textbf{Q1}, the fingertip information from motion capture dataset, when faced with a large embodiment gap and dynamic tasks, can lead to inaccurate contact information. Thus this information provide incorrect constraints in the policy learning. Additionally, considering the difficulty of acquiring fingertip information in real-world robots, we cannot include fingertips position in the observations, which also may is a reason of the poor outcomes when with the fingertip rewards.

\textbf{Q5: What effect does Data Augmentation Loop in DexMimic?}
In Table 1 and Table 4, The policy with DAL are all better than those without DAL. Figure 5(b) illustrates the performance improvement of adding three type of randomizations in the task. Only with a maximum allowance of four iteration times, Ours can improve more than $30\%$ in completion rate. This result concludes that DAL makes the trained policy better against disturbance, which is a more robust policy.

\textbf{Q6: How well does our method perform on dexterous robotic hands other than the Shadow Hand?}
In Figure 5(c), we conducted experiments on task-level retargeting with four types of hands, achieving an average completion rate of 80\%. This demonstrates that our framework can be effectively applied to various types of hands. The results show that the Allegro Hand performed the worst, followed by the Ability Hand and Schunk Hand, with the Shadow Hand performing the best. This indicates that higher degrees of freedom and a smaller embodiment gap with the human hand both lead to better task-level retargeting results, aligning with the expectations.

\textbf{Q7: Can our policy be transferred from simulation to real-world robots?}

In Table 3 real-world experiments, our approach has more than 30\% success rate improvements compared to prior methods. This result is consistent with the results in simulation. Ours has a more than $6\%$ success rate in all of the task, while the other baselines have a $0\%$ success rate in most of the task. This result highlights the ability of our model when tackling task-level retargeting in the real-world. For more details of the real-world setups, please refer to Appendix.~\ref{app:real_implement}.

==> table_1.tex <==
\begin{figure}

\begin{minipage}[!t]{0.48\textwidth}

\centering
\begin{tabular}{c|c|ccc}
\toprule
                             &         & BC     & BC-RNN & Ours  \\ \midrule
\multirow{2}{*}{Trained}     & TE & 5.4   &   5.0     & \textbf{4.2}       \\
                             & OE & 14.6  &    12.4    & \textbf{9.6}        \\ \midrule
Unseen & TE & 5.6   &  6.2      & \textbf{5.0}      \\
Traj                             & OE & 9.4   &   9.2     & \textbf{7.2}      \\ \midrule
Unseen  & TE & 18.2  &    17.7    & \textbf{12.4}      \\
Object                             & OE & 109.4 &     82.2   & \textbf{75.5}      \\
\bottomrule

\end{tabular}
% \vspace{5pt}
\captionof{table}{Results for the high-level planner}
\label{tab:table_1}

\end{minipage}
\hspace{0.2cm}
\begin{minipage}[!t]{0.48\textwidth}

\centering
\label{tab:my-table}
\begin{tabular}{l|cccc}
\toprule
& \multirow{2}{*}{\shortstack{Fingertip \\ Mapping}} & \multirow{2}{*}{\shortstack{Vanilla \\RL}} & \multirow{2}{*}{Ours} \\
 &   
  \\
\midrule
Box               & 15.2         & 22.1       &  \textbf{70.1}  \\
Microwave         &   62.1       &   57.7     &  \textbf{100} \\
Laptop            & 9.2         & 10.2       & \textbf{81.2}   \\
Coffee Maker    & 10.4         & 11.4       & \textbf{75.2}   \\
Mixer             & 17.5         &  20.2      & \textbf{91.7}   \\
Notebook          &    4.5      &    4.5    &   \textbf{69.9} \\
\bottomrule

\end{tabular}
% \vspace{5pt}
\captionof{table}{Results for the real-world experiments}
\label{tab:table_2}

\end{minipage}
\vspace{-0.3cm}

\end{figure}

==> table_1_var.tex <==
\begin{figure}

\begin{minipage}[!t]{0.48\textwidth}

\centering
\begin{tabular}{c|c|ccc}
\toprule
                             &         & MLP     & RNN & Ours  \\ \midrule
\multirow{2}{*}{Trained}     & TE & \pms{5.4}{0.2}   &   \pms{5.0}{0.1}     & \pms{\textbf{4.2}}{0.2}       \\
                             & OE & \pms{14.6}{0.7}  &    \pms{12.4}{0.8}    & \pms{\textbf{9.6}}{0.6}        \\ \midrule
Unseen & TE & \pms{5.6}{0.5}   & \pms{6.2}{0.3}      & \pms{\textbf{5.0}}{0.8}      \\
Traj                             & OE & \pms{9.4}{1.0}   &   \pms{9.2}{0.5}     & \pms{\textbf{7.2}}{0.7}      \\ \midrule
Unseen  & TE & \pms{18.2}{1.5}  &    \pms{17.7}{1.2}    & \pms{\textbf{12.4}}{1.1}      \\
Object                             & OE & \pms{109.4}{5.8} &     \pms{82.2}{4.2}   & \pms{\textbf{75.5}}{4.7}      \\
\bottomrule

\end{tabular}
% \vspace{5pt}
\captionof{table}{Results for the high-level planner}
\label{tab:table_1}

\end{minipage}
\hspace{0.2cm}
\begin{minipage}[!t]{0.48\textwidth}

\centering
\label{tab:my-table}
\begin{tabular}{l|cccc}
\toprule
& \multirow{2}{*}{\shortstack{Fingertip \\ Mapping}} & \multirow{2}{*}{\shortstack{Vanilla \\RL}} & \multirow{2}{*}{Ours} \\
 &   
  \\
\midrule
Box               & \pms{15.2}{2.7}         & \pms{22.1}{1.2}       &  \pms{\textbf{70.1}}{5.3}  \\
Microwave         &   \pms{62.1}{7.1}       &   \pms{57.7}{10.2}     &  \pms{\textbf{100}}{0.0} \\
Laptop            & \pms{9.2}{0.5}         & \pms{10.2}{0.9}       & \pms{\textbf{81.2}}{6.1}   \\
Coffee M.    & \pms{10.4}{0.3}         & \pms{11.4}{1.4}       & \pms{\textbf{75.2}}{4.8}   \\
Mixer             & \pms{17.5}{1.7}         &  \pms{20.2}{2.2}      & \pms{\textbf{91.7}}{5,5}   \\
Notebook          &    \pms{4.5}{0.1}      &    \pms{4.5}{0.3}    &   \pms{\textbf{69.9}}{12.6} \\
\bottomrule

\end{tabular}
% \vspace{5pt}
\captionof{table}{Results for the real-world experiments}
\label{tab:table_2}

\end{minipage}
\vspace{-0.3cm}

\end{figure}

==> table_2.tex <==
\begin{table}[!t]
\centering
\tiny
\begin{tabular}{l|ccccccccc}
\toprule
 % &
 %  Box &
 %  Capsule &
 %  Espresso &
 %  Ketch &
 %  Micro &
 %  Mixer &
 %  Note &
 %  Scis &
 %  % Waffle &
 %  Laptop \\
 % &
 %   &
 %  Machine &
 %  Machine &
 %  up &
 %  wave &
 %   &
 %  book &
 %  sors &
 %  % iron &
  
& \multirow{2}{*}{Box} & \multirow{2}{*}{\shortstack{Coffee \\ Maker}} & \multirow{2}{*}{\shortstack{Espresso \\Machine}} & \multirow{2}{*}{Ketch} & \multirow{2}{*}{\shortstack{Micro- \\ wave}} & \multirow{2}{*}{Mixer} & \multirow{2}{*}{\shortstack{Note- \\ book}} & \multirow{2}{*}{\shortstack{Scis- \\ sors}} & \multirow{2}{*}{Laptop}

   \\ \\
  
\midrule
Fingertip Mapping &

  \multicolumn{1}{r}{\pms{15.2}{0.1}} &
  \multicolumn{1}{r}{\pms{11.7}{0.8}} &
  \multicolumn{1}{r}{\pms{33.7}{0.2}} &
  \multicolumn{1}{r}{\pms{16.5}{0.1}} &
  \multicolumn{1}{r}{\pms{41.8}{0.7}} &
  \multicolumn{1}{r}{\pms{22.6}{0.9}} &
  \multicolumn{1}{r}{\pms{12.3}{0.4}} &
  \multicolumn{1}{r}{\pms{5.1}{0.2}} &
  % \multicolumn{1}{r}{7.7} &
  \multicolumn{1}{r}{\pms{11.1}{0.4}} \\
Finger Joint Mapping &
  \multicolumn{1}{r}{\pms{10.0}{0.4}} &
  \multicolumn{1}{r}{\pms{10.7}{0.7}} &
  \multicolumn{1}{r}{\pms{9.7}{0.4}} &
  \multicolumn{1}{r}{\pms{12.5}{0.5}} &
  \multicolumn{1}{r}{\pms{31.7}{0.4}} &
  \multicolumn{1}{r}{\pms{13.8}{0.6}} &
  \multicolumn{1}{r}{\pms{7.9}{0.1}} &
  \multicolumn{1}{r}{\pms{6.2}{0.1}} &
  % \multicolumn{1}{r}{7.7} &
  \multicolumn{1}{r}{\pms{10.6}{1.7}} \\
Vanilla RL &
  \multicolumn{1}{r}{\pms{26.8}{1.4}} &
  \multicolumn{1}{r}{\pms{11.6}{0.8}} &
  \multicolumn{1}{r}{\pms{15.1}{0.7}} &
  \multicolumn{1}{r}{\pms{6.9}{1.7}} &
  \multicolumn{1}{r}{\pms{46.6}{2.2}} &
  \multicolumn{1}{r}{\pms{46.4}{1.1}} &
  \multicolumn{1}{r}{\pms{12.8}{0.9}} &
  \multicolumn{1}{r}{\pms{5.7}{0.0}} &
  % \multicolumn{1}{r}{7.7} &
  \multicolumn{1}{r}{\pms{37.6}{4.5}} \\
Ours (w. FR) &
  \multicolumn{1}{r}{\pms{59.3}{8.1}} &
  \multicolumn{1}{r}{\pms{80.3}{2.1}} &
  \multicolumn{1}{r}{\pms{84.2}{4.1}} &
  \multicolumn{1}{r}{\pms{21.0}{3.8}} &
  \multicolumn{1}{r}{\pms{65.2}{2.9}} &
  \multicolumn{1}{r}{\pms{43.9}{5.1}} &
  \multicolumn{1}{r}{\pms{34.1}{5.8}} &
  \multicolumn{1}{r}{\pms{23.9}{1.2}} &
  % \multicolumn{1}{r}{7.7} &
  \multicolumn{1}{r}{\pms{44.7}{7.7}} \\
Ours (w.o. DAL)&
  \multicolumn{1}{r}{\pms{100}{0.0}} &
  \multicolumn{1}{r}{\pms{74.8}{4.2}} &
  \multicolumn{1}{r}{\pms{89.6}{3.5}} &
  \multicolumn{1}{r}{\pms{27.3}{6.8}} &
  \multicolumn{1}{r}{\pms{100}{0.0}} &
  \multicolumn{1}{r}{\pms{47.1}{5.5}} &
  \multicolumn{1}{r}{\pms{39.4}{4.7}} &
  \multicolumn{1}{r}{\pms{37.8}{5.2}} &
  % \multicolumn{1}{r}{61.0} &
  \multicolumn{1}{r}{\pms{100}{0.0}} \\
Ours &
  \multicolumn{1}{r}{\pms{\textbf{100}}{0.0}} &
  \multicolumn{1}{r}{\pms{\textbf{88.1}}{6.2}} &
  \multicolumn{1}{r}{\pms{\textbf{91.2}}{7.9}} &
  \multicolumn{1}{r}{\pms{\textbf{44.5}}{12.0}} &
  \multicolumn{1}{r}{\pms{\textbf{100}}{0.0}} &
  \multicolumn{1}{r}{\pms{\textbf{61.1}}{4.2}} &
  \multicolumn{1}{r}{\pms{\textbf{40.1}}{4.3}} &
  \multicolumn{1}{r}{\pms{\textbf{42.4}}{19.6}} &
  % \multicolumn{1}{r}{$\bm{71.5}$} &
  \multicolumn{1}{r}{\pms{\textbf{100}}{0.0}} \\
  \bottomrule
\end{tabular}
\vspace{5pt}
\caption{Results for the experiments of using one policy per object.}
\label{tab:table_3}

\vspace{-0.5cm}
\end{table}

==> table_2_inverse.tex <==
\begin{table}[t]
\centering
% \small
\begin{tabular}{l|cccccc}
\toprule
 % &        & Finger & Joint & Vanilla & Ours        & Ours & Ours \\
 %  &        & IK & IK & RL & (w. FR)       & (w.o. PCIL)    &

& \multirow{2}{*}{\shortstack{Fingertip \\ Mapping}} & \multirow{2}{*}{\shortstack{Finger Joint \\ Mapping}} & \multirow{2}{*}{\shortstack{Vanilla \\RL}} & \multirow{2}{*}{\shortstack{Ours \\ (w. FR)}} & \multirow{2}{*}{\shortstack{Ours \\ (w.o. DAL)}} & \multirow{2}{*}{Ours} \\
 &   
  \\ \midrule
Box & \pms{15.2}{0.1} & \pms{10.0}{0.4} & \pms{26.8}{1.4} & \pms{59.3}{8.1} &  \pms{100}{0.0} & \pms{\textbf{100}}{0.0} \\

Coffee Maker & \pms{11.7}{0.8}    & \pms{10.7}{0.7}    & \pms{11.6}{0.8}    & \pms{80.3}{2.1}               & \pms{74.8}{4.2} & \pms{\textbf{88.1}}{6.2} \\

Espresso Machine& \pms{33.7}{0.2}      & \pms{9.7}{0.4}  & \pms{15.1}{0.7} & \pms{84.2}{4.1} &  \pms{89.6}{3.5}       & \pms{\textbf{91.2}}{7.9} \\

Ketchup& \pms{16.5}{0.1}   & \pms{12.5}{0.5}    & \pms{6.9}{1.7}    & \pms{21.0}{3.8}       & \pms{27.3}{6.8}       & \pms{\textbf{44.5}}{12.0} \\

Microwave & \pms{41.8}{0.7} & \pms{31.7}{0.4} & \pms{46.6}{2.2} & \pms{65.2}{2.9} &  \pms{100}{0.0} & \pms{\textbf{100}}{0.0} \\

Mixer & \pms{22.6}{0.9}    & \pms{13.8}{0.6}    & \pms{46.4}{1.1}    & \pms{43.9}{5.1}               & \pms{47.1}{5.5} & \pms{\textbf{61.1}}{4.2} \\

Notebook& \pms{12.3}{0.4}       & \pms{7.9}{0.1}  & \pms{12.8}{0.9} & \pms{34.1}{5.8} &  \pms{39.4}{4.7}       & \pms{\textbf{40.1}}{4.3} \\

Scissors & \pms{5.1}{0.2}   & \pms{6.2}{0.1}    & \pms{5.7}{0.0}    & \pms{23.9}{1.2}       & \pms{37.8}{5.2}       & \pms{\textbf{42.4}}{19.6} \\

Laptop & \pms{11.1}{0.4}   & \pms{10.6}{1.7}    & \pms{37.6}{4.5}    & \pms{44.7}{7.7}       & \pms{100}{0.0}       & \pms{\textbf{100}}{0.0} \\

\bottomrule
\end{tabular}
\vspace{5pt}
\caption{Results for the generalization experiments.}
\label{tab:table_3}
\vspace{-0.5cm}
\end{table}

==> table_3.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{l|cccccc}
\toprule
 % &        & Finger & Joint & Vanilla & Ours        & Ours & Ours \\
 %  &        & IK & IK & RL & (w. FR)       & (w.o. PCIL)    &

& \multirow{2}{*}{\shortstack{Fingertip \\ Mapping}} & \multirow{2}{*}{\shortstack{Finger Joint \\ Mapping}} & \multirow{2}{*}{\shortstack{Vanilla \\RL}} & \multirow{2}{*}{\shortstack{Ours \\ (w. FR)}} & \multirow{2}{*}{\shortstack{Ours \\ (w.o. DAL)}} & \multirow{2}{*}{Ours} \\
 &   
  \\ \midrule
% Single Obj - Trained Traj & 12.1 & 8.6 & 18.4 & 31.5 &  61.1 & $\bm{85.7}$ \\
% Single Obj - Unseen Traj & -    & -    & 20.3    & -               & 44.1 & $\bm{60.6}$ \\ \midrule 
% Multi Obj - Trained Obj& 8.3       & 6.3  & 19.4 & 17.2 &  37.1       & $\bm{51.2}$ \\
%  Multi Obj - Unseen Obj& -   & -    & 10.2    & -       & 20.2       & $\bm{38.6}$ \\
Single Obj - Trained Traj& \pms{12.1}{4.2} & \pms{8.6}{5.2} & \pms{18.4}{10.8} & \pms{31.5}{15.3} &  \pms{61.1}{17.6} & \pms{\textbf{85.7}}{10.1} \\
Single Obj - Unseen Traj& \pms{5.3}{0.2}    & \pms{6.1}{0.3}    & \pms{20.3}{9.2}    & \pms{21.1}{12.6}               & \pms{44.1}{9.2} & \pms{\textbf{60.6}}{8.8} \\ \midrule 
Multi Obj - Trained Obj& \pms{8.3}{2.1}       & \pms{6.3}{3.4}  & \pms{19.4}{12.2} & \pms{17.2}{5.8} &  \pms{37.1}{3.7}       & \pms{\textbf{51.2}}{6.0} \\
 Multi Obj - Unseen Obj& \pms{3.7}{0.8}   & \pms{2.9}{0.2}    & \pms{10.2}{7.4}    & \pms{9.3}{4.1}       & \pms{20.2}{5.2}       & \pms{\textbf{38.6}}{6.9} \\
\bottomrule
\end{tabular}
\vspace{5pt}
\caption{Results for the generalization experiments.}
% \caption{Results for the genaralization experiments. Multi Traj means using one policy to solve the task-level retargeting of multiple trajectories, and generalizing to unseen trajectories. Multi Obj means using one policy to solve the task-level retargeting of multiple objects, and generalizing to unseen objects. The number in the table is the completion rate.}
\label{tab:table_4}
\vspace{-1.0cm}
\end{table}
